Synthesizing Specifications

Every program should be accompanied by a specification that describes important aspects of the code's behavior, but writing good specifications is often harder than writing the code itself. This paper addresses the problem of synthesizing specifications automatically, guided by user-supplied inputs of two kinds: i) a query posed about a set of function definitions, and ii) a domain-specific language L in which the extracted property is to be expressed (we call properties in the language L-properties). Each of the property is a best L-property for the query: there is no other L-property that is strictly more precise. Furthermore, the set of synthesized L-properties is exhaustive: no more L-properties can be added to it to make the conjunction more precise. We implemented our method in a tool, Spyro. The ability to modify both the query and L provides a Spyro user with ways to customize the kind of specification to be synthesized. We use this ability to show that Spyro can be used in a variety of applications, such as mining program specifications, performing abstract-domain operations, and synthesizing algebraic properties of program modules.

==> with_vs_without_minimization_plot.tex <==
\begin{tikzpicture}[]
  \tikzset{mark options={mark size=1, opacity=0.3}}
  \begin{axis}[
    title={\small Not minimized vs. Minimized $\eminusmust$.},
    xlabel style={yshift=1mm},
    ylabel style={yshift=-3mm},
    height=0.95\linewidth,
    width=0.95\linewidth,
    xlabel= {\small Not minimized (s)}, ylabel= {\small Minimized (s)},
    %scaled x ticks=base 10:-3,scaled y ticks=base 10:-3,
    xtick scale label code/.code={},ytick scale label code/.code={}
  ]
  \addplot+[only marks]
table {
195.57	282.54
26.96	38.67
207.88	256.93
39.75	50.72
643.76	557.4
70.93	87.64
196.92	295.94
14.12	19.08
51.06	91.78
185.45	274.32
220.58	316.36
206.5	337.68
232.93	323.27
158.38	225.7
44.16	61.25
144.3	194.22
104.31	148.84
30.48	41.28
41.59	67.08
212.49	310.04
47.7	70.13
173.16	190.06
68.01	92.92
95.76	143.38
400.87	570.04
22.39	29.47
441.48	513.77
14.53	28.34
27.69	55.71
240.08	355.85
26.6	53.78
388.92	494.19
395.52	545.71
248.83	331.85
3376.82	4519.83
68.1	105.62
15.64	22.95
92.31	106.65
892.6	661.34
499.09	498.07
228.6	231.36
29.72	31.7
83.11	106.64
744.03	1513.94
9042.73	5626.71
};
\draw [solid, color=red] (-100, -100) -- (600,600);
\end{axis}
\end{tikzpicture}

